Beyond Sequence Order: Syntax-Informed Positional Embeddings for Transformers

Positional embeddings (PE) in Transformers encode token distance and order but are largely agnostic to \textit{syntactic structure}. We introduce \textbf{S}yntax-\textbf{i}nformed \textbf{P}ositional \textbf{E}mbeddings (\textbf{SiPE}), which learns a lightweight syntactic prior from dependency parses during pretraining and injects it across all three dominant PE families (absolute, relative, rotary), for both encoders and decoders, leaving self-attention and the rest of the architecture untouched. We isolate \emph{where} and \emph{how} the prior should enter the model, and find it depends on the architecture: for autoregressive decoders that use relative PE, the prior is strongest when coupled multiplicatively with the relative-position term of the attention score, outperforming injection into the input embeddings, into self-attention, or into the positional and attention terms jointly---while for encoders it is best added directly to the input embeddings, composing with each encoder's native positional mechanism. We find that models pre-trained with SiPE improve on the SyntaxGym benchmark by up to $10.3\%$ while simultaneously reducing perplexity by $9.0\%$ over a base model with no syntactic supervision---a metric nearly every existing syntax-injection method instead degrades. Crucially, these gains extend beyond syntactic generalization: SiPE also improves real-world language understanding, raising scores on the GLUE benchmark by up to $8.2\%$ over a model trained without it. Unlike existing syntactic language models that marginalize over many parses at inference or discard syntax at runtime, SiPE conditions on a single parse, establishing a new Pareto frontier between syntactic supervision and inference cost.

==> sections/inference-pareto.tex <==
\section{Moving the Pareto-frontier of Syntactic Language Models}
\label{sec:top_parse_approx}

% Joint syntactic LMs such as PLM~\cite{qian-etal-2021-structural}, Transformer Grammars~\cite{Sartran_2022}, Pushdown LMs~\cite{murty2023pushdownlayersencodingrecursive}, and DTG~\cite{zhao2024dependencytransformergrammarsintegrating} factorize $p(x, y)$ over tokens and syntactic structures, then recover $p(x)$ by marginalizing over $y \in \mathcal{Y}$. In practice, this marginal is approximated by enumerating hundreds of candidate trees via word-synchronous beam search~\cite{stern-etal-2017-effective,crabbe-etal-2019-variable} or an external parser~\cite{Yoshida_2024}, multiplying inference cost by $|\mathcal{Y}|$ on top of the parser's own overhead.

% We sidestep this with a single-parse approximation: at inference, we condition on the top-scoring parse $(\hat{\boldsymbol{\tau}}, \hat{\boldsymbol{\nu}})$ from a trained \texttt{DeBERTa-v3-base} hexatagger instead of marginalizing,
% %
% \begin{equation}
% p(x) \;\approx\; p\bigl(x \mid \hat{\boldsymbol{\tau}}, \hat{\boldsymbol{\nu}}\bigr).
% \label{eq:top_parse}
% \end{equation}
% %
% The model then behaves as an ordinary LM at both training and inference: hexatags are additional inputs, no beam search is required, and inference cost reduces to the LM forward pass plus a single linear-time parse --- roughly $300\times$ cheaper than approaches requiring marginalization. We argue this is a worthwhile trade. We outperform parser-free methods (TreeReg \cite{nandi2025sneakingsyntaxtransformerlanguage}, TPT \cite{Yoshida_2024}) on both SyntaxGym and perplexity (\autoref{tab:results_delta-dup1}), and while methods which do use parsers and jointly model syntax with language do slightly outperform ours on BLIMP and SG, our $300\times$ inference cost reduction --- one parse per sentence vs.\ marginalization over hundreds --- makes the trade favorable in any setting where inference cost matters.

Joint syntactic LMs such as PLM~\cite{qian-etal-2021-structural}, Transformer Grammars~\cite{Sartran_2022}, Pushdown LMs~\cite{murty2023pushdownlayersencodingrecursive}, and DTG~\cite{zhao2024dependencytransformergrammarsintegrating} factorize $p(x, y)$ over tokens and syntactic structures, then recover $p(x) = \sum_{y \in \mathcal{Y}} p(x, y)$ by marginalizing over $\mathcal{Y}$ --- in practice approximated by enumerating hundreds of candidate trees via word-synchronous beam search~\cite{stern-etal-2017-effective,crabbe-etal-2019-variable} or an external parser~\cite{Yoshida_2024}, multiplying inference cost by $|\mathcal{Y}|$.

We sidestep this with a single-parse approximation: at inference, we condition on the top-scoring parse from a trained \texttt{DeBERTa-v3-base} hexatagger, $p(x) \approx p(x \mid \hat{\boldsymbol{\tau}}, \hat{\boldsymbol{\nu}})$. The model then behaves as an ordinary LM: hexatags are additional inputs, no beam search is required, and inference cost reduces to the LM forward pass plus a single linear-time parse --- roughly $300\times$ cheaper. We outperform parser-free methods (TreeReg~\cite{nandi2025sneakingsyntaxtransformerlanguage}, TPT~\cite{Yoshida_2024}) on both SyntaxGym and perplexity (\autoref{tab:results_delta-dup1}); and while methods which do use parsers and jointly model syntax with language do slightly outperform ours on BLIMP and SG, our $300\times$ inference cost reduction makes this trade-off favorable wherever inference cost matters.
